Beyond Perturbation Stability: LP Recovery Guarantees for MAP Inference on Noisy Stable Instances

Several works have shown that perturbation stable instances of the MAP inference problem in Potts models can be solved exactly using a natural linear programming (LP) relaxation. However, most of these works give few (or no) guarantees for the LP solutions on instances that do not satisfy the relatively strict perturbation stability definitions. In this work, we go beyond these stability results by showing that the LP approximately recovers the MAP solution of a stable instance even after the instance is corrupted by noise. This "noisy stable" model realistically fits with practical MAP inference problems: we design an algorithm for finding "close" stable instances, and show that several real-world instances from computer vision have nearby instances that are perturbation stable. These results suggest a new theoretical explanation for the excellent performance of this LP relaxation in practice.

==> Paper/related.tex <==
\subsection{Related work.}
\paragraph{Perturbation stability.}
Several works have given recovery guarantees for the local LP relaxation on perturbation stable instances of uniform metric labeling \citep{LanSonVij18, LanSonVij19} and for similar problems \citep{makarychev2014bilu, AngMakMak17}.
%Aside from \citet{LanSonVij19}, none of these works gives a guarantee for the local LP relaxation when the observed instance $\obsins$ does not satisfy the strict stability assumptions (that are  not satisfied in practice). \citet{LanSonVij19} give partial recovery guarantees for the local LP when parts (blocks) of the observed instance satisfy a stability-like condition (that involves the dual program on the instance), and they showed that practical instances have ``blocks'' that satisfy their condition. We take a different approach in this work: we do not make any explicit assumptions involving the linear program (or its dual) for the observed instance $\obsins$. Instead, we merely assume this instance is ``close'' to a latent stable instance $\stabins$, but we are still able to give partial recovery guarantees for the local LP. Our empirical results also indicate that real-world instances are close to stable.
Finally, \citet{makarychev2014bilu} consider a notion of weak stability for graph partitioning problems, where the optimal solution is allowed to change a bit under perturbations. However, their guarantees are for a different algorithm, and do not explain the performance of the linear programming relaxation. 

\paragraph{Easy instances corrupted with noise.}
Our random noise model is similar to several planted average-case models like stochastic block models (SBMs) considered in the context of problems like community detection, correlation clustering and partitioning \citep[see e.g.,][]{Mcsherry,Abbesurvey, GRSY15}. Instances generated from these models can also be seen as the result of random noise injected into an instance with a nice block structure that is easy to solve. 
Several works give exact recovery and approximate recovery guarantees for semidefinite programming (SDP) relaxations for such models in different parameter regimes~\cite{Abbesurvey,guedon2016community}. 
In our model however, we start with an {\em arbitrary} stable instance as opposed to an instance with a block structure (which is trivial to solve). 
Moreover, we are unaware of such analysis in the context of linear programs.
Please see Section~\ref{sec:random-model} for a more detailed comparison. To the best of our knowledge, we are the first to consider study instances generated from random perturbations to stable instances.
